HiDAnet: RGB-D Salient Object Detection via Hierarchical Depth Awareness

RGB-D saliency detection aims to fuse multi-modal cues to accurately localize salient regions. Existing works often adopt attention modules for feature modeling, with few methods explicitly leveraging fine-grained details to merge with semantic cues. Thus, despite the auxiliary depth information, it is still challenging for existing models to distinguish objects with similar appearances but at distinct camera distances. In this paper, from a new perspective, we propose a novel Hierarchical Depth Awareness network (HiDAnet) for RGB-D saliency detection. Our motivation comes from the observation that the multi-granularity properties of geometric priors correlate well with the neural network hierarchies. To realize multi-modal and multi-level fusion, we first use a granularity-based attention scheme to strengthen the discriminatory power of RGB and depth features separately. Then we introduce a unified cross dual-attention module for multi-modal and multi-level fusion in a coarse-to-fine manner. The encoded multi-modal features are gradually aggregated into a shared decoder. Further, we exploit a multi-scale loss to take full advantage of the hierarchical information. Extensive experiments on challenging benchmark datasets demonstrate that our HiDAnet performs favorably over the state-of-the-art methods by large margins.

==> blabla.tex <==

\begin{table*}[t]
\scriptsize
\setlength\tabcolsep{4.3pt}
\setlength\extrarowheight{1pt}
\begin{center}
\caption{\textbf{Quantitative comparison} with SOTA models. $\uparrow$ ($\downarrow$) denotes that the higher (lower) is better. (\bl{Bold}: best.)}
\label{tab:quant}
\begin{tabular*}{\linewidth}{ll|| llll|llll|llll|llll|llll}
 \hline 

\hline

\hline
 Dataset &Size  &\multicolumn{4}{c}{DES} & \multicolumn{4}{c}{NLPR}  & \multicolumn{4}{c}{NJU2K}  & \multicolumn{4}{c}{STERE} & \multicolumn{4}{c}{SIP}  \\%& \multicolumn{4}{c}{SSD} \\
\cline{3-6} \cline{7-10} \cline{11-14} \cline{15-18} \cline{19-22} %\cline{22-25}

Metric & Mb & $M\downarrow$ &  $F_{\beta}\uparrow $  &  $S_m\uparrow$ &  $E_m\uparrow$  &  $M\downarrow$ &  $F_{\beta}\uparrow $  &  $S_m\uparrow$ &  $E_m\uparrow$  &  $M\downarrow$ &  $F_{\beta}\uparrow $  &  $S_m\uparrow$ &  $E_m\uparrow$  &  $M\downarrow$ &  $F_{\beta}\uparrow $  &  $S_m\uparrow$ &  $E_m\uparrow$  &  $M\downarrow$ &  $F_{\beta}\uparrow $  &  $S_m\uparrow$ &  $E_m\uparrow$  \\%&  $M\downarrow$ &  $F_{\beta}\uparrow $  &  $S\uparrow$ &  $E\uparrow$\\
\hline
%$CPFP_{19}$ & .038 & .846 & .872  &.923 & .036 & .867 & .888  &.932 & .053 & .877 & .878  &.923 & .051 & .874 & .879  &.925 & .064 & .851 & .850  &.903 \\%& .082 & .766 & .807  &.852 \\

\multicolumn{15}{l}{\textbf{Performance of RGB-D Models with VGG Backbones}} \\

$DMRA_{19}$ \cite{piao2019dmra} & 278& .030 & .907 & .900 &.934 & .031 & .888 & .899 &.940 
                                & .051 & .896 & .886 &.920 
                                & .047 & .895 & .886 &.930
                                & .086 & .852 & .806 &.847  \\% & .058 & .844 & .857  &.906 \\
$A2dele_{20}$ \cite{piao2020a2dele} & 116 & .029 & .897 & .886  &.917 & .029 & .895 & .899  &.943 & .051 & .890 & .871  &.914 & .044 & .892 & .879  &.926 & .070 & .856 & .829  &.887 \\%& .070 & .776 & .802  &.861 \\

$ATSA_{20}$ \cite{zhang2020asymmetric}& 131  & .022 & .931 & .917  &.954 & .027 & .907 & .909  &.947 & .046 & .905 & .885  &.928 & .038 & .912 & .896  &\textbf{.940} & .063 & .884 & .849  &.895 \\%& .070 & .776 & .802  &.861 \\

$CMMS_{20}$ \cite{li2020rgb}& 546  & .018  & .934 & .934  &.958 & .028 & .914 & .919  &.946 & .044 & .905 & .900  &.929 & .045 & .899 & .894  &.925 & .058 & .893 & .872  &.901 \\%& .046 & .874 & .864  &.922 \\
$DANet_{20}$ \cite{zhao2020single}& 128  & .029 & .916 & .904 &.932 & .047 & .904 & .897 &.926 
                                & .045 & .910 & .899 & .927
                                & .048 & .895 & .892 &.919 
                                & .054 & .900 & .888 &.912 \\%& .050 & .866 & .864  &.914 \\


$CMWNet_{20}$ \cite{li2020cross}  & 327 & .022 & .939 & .934  &.959 & .029 & .913 & .917  &.941 & .046 & .913 & .903  &.925 & .043 & .911 & .905  &.930 & .062 & .889 & .867  &.901 \\%& .068 & .795 & .830  &.885 \\

$HDFNet_{20}$ \cite{pang2020hierarchical}& 308 & .021 & .932 & .926  &.962 & .023 & .926 & .923  &.957 & .039 & .922 & .908  &.939 & .042 & .910 & .900  &.933 &.048 & \textbf{.909} & .886  &.924 \\%& .048 & .808 & .866  &.913\\                      

$PGAR_{20}$ \cite{chen2020progressively}& 62 & .032 & .894 & .886  &.906 & .027 & .912 & .917  &.941 & .042 & .918 & .909  &.932 & .045 & .902 & .894  &.919 &.072 & .852 & .838  &.875 \\%& .048 & .808 & .866  &.913\\      

$SSF_{20}$ \cite{zhang2020select} & 126 & .026 & .912 & .904  &.930 & .027 & .912 & .915  &.947 & .043 & .911 & .899  &.929 & .065 & .859 & .837  &.882 &.091 & .810 & .799  &.855 \\%& .048 & .808 & .866  &.913\\

$CASGNN_{20}$ \cite{luo2020cascade}& 160  & .027 & .917 & .893  &.926 & .025 & .914 & .919  &.953 & .036 & .927 & .910  &.944 & \textbf{.038} & .913 & .899  &\textbf{.940} & -& - & -  &- \\%& .044 & .859 & .882  &.919 \\

$D3Net_{21}$ \cite{fan2019rethinkingd3}& 518 & .031 & .909 & .897 &.923 & .030 & .907 & .912 &.942 
                                & .049 & .910 & .900 &.928 
                                & .039 & .911 & .902 &\textbf{.940} 
                                & .063 & .886 & .866 &.897\\%& .058 & .834 & .857  &.910 \\
$CDINet_{21}$ \cite{CDINet} & 217 & .020 & .943 & \bl{.937} &.962 & .024 & .923 & .927 &.953 
                                & \textbf{.030} & .928 & \textbf{.918} &.945 
                                & .040 & .912 & \textbf{.913} &.937 
                                & .054 & .904 & .875 &.908 \\%& - & - & -  & - \\

$UCNet_{21}$ \cite{zhang2021uncertainty} & 120 & .018 & .936 & .934 & \textbf{.970} &.025 & .915 & .920 & .953 & .043 & .908 & .897 & .932 & .039 & .908 & .902 &.938 & .051 & .896 & .875 & .915\\ 
$DRLF_{21}$ \cite{wang2020data} & 351 & .030 & .909 & .895  &.918 & .032 & .904 & .903  &.929 & .055 & .896 & .886  &.914 & .050 & .897 & .888  &.916 & .071 & .869 & .850  &.882 \\%& .068 & .795 & .830  &.885 \\
$HAINet_{21}$ \cite{li2021hierarchical}  & 228 & .018 & \textbf{.945} & .935  &.967 &  .024&   .920&   .924&   .956 
                                      &  .037&   .924&   .911&   .940
                                      &  .040&   \textbf{.917}&   .907&   .938 
                                      &  .052&   .907&   .879&   .917 \\
$DCMF_{22}$ \cite{wang2022learning} & 78& .022 & .934 & .932 & .956  &.029 & .913 & .922 & .940 & .041  & .911 &  .902 & .935 & .043 & .916 & .910 & .928 & - & -& -& -\\ 

\rowcolor[RGB]{235,235,250} 
\textbf{Ours (VGG16)} & 269 & \textbf{.017} & .944 & .929 & .968  &\textbf{.021} & \textbf{.927} & \textbf{.928} & \textbf{.962} & .034 & \textbf{.930 }& \textbf{.918} & \textbf{.947} & .039 & .915 & .902 & .939 & \textbf{.045} & \textbf{.909} & \textbf{.889} & \textbf{.927} \\

\hline
\multicolumn{15}{l}{\textbf{Performance of RGB-D Models with ResNet Backbones}} \\
$JLDCF_{21}$ \cite{fu2021siamese} & 548 & .020 & .934 & .931  &.961 & .022 & .925 & .925  &.955 & .041 & .912 & .902  &.936 & .040 & .913 & .903  &.934 & .049 & .903 & .880  &.918 \\%& .068 & .795 & .830  &.885 \\

$RD3D_{21}$ \cite{chen2021rgb}  & 179 & .019 & .941 & .935  &.965 & .022 & .927 & .930  &.959 & .036 & .923 & .916  &.941 & - &- & -  &- & .091 & .816 & .803  &.848 \\%& .068 & .795 & .830  &.885 \\


$BIANet_{21}$ \cite{zhang2021bilateral} & 244 & .038 & .868 & .861  &.874 & .033 & .889 & .900  &.931 & .056 & .879 & .868  &.899 & .037 & .917 & .911  &.939 & .048 & .906 & .885  &.918 \\%& .068 & .795 & .830  &.885 \\





$CoNet_{20}$ \cite{ji2020accurate}& 162 & .024 & .920 & .914  &.944 & .027 & .903 & .911  &.943 & .046 & .902 & .896  &.926 & .037 & .909 & .905  &.941 & .058 & .887 & .860  &.911\\% & .059 & .840 & .853  &.915 \\

$DASNet_{20}$ \cite{zhao2020depth} & 141 & .024 & .926 & .905  &.932 & .021 & \bl{.929} & .929  &.960 & .042 & .911 & .902  &.935 & .037 & .915 & .910  &.939 &.051 & .900 & .877  &.918 \\%& .042 & .881 & .885  &- \\


$BBSNet_{21}$ \cite{zhai2021bifurcated}& 200 & .021 & .942 & .934  &.955 & .023 & .927 & .930  &.953 & .035 & .931 & .920  &.941 & .041 & .919 & .908  &.931 &.055 & .902 & .879  &.910 \\%& .044 & .859 & .882  &.919 \\

$DCF_{21}$ \cite{ji2021calibrated} & 435 & .024 &.910 & .905 &.941   &  .022&   .918&   .924&   .958
                                      &  .036&   .922&   .912&   .946
                                      &  .039&   .911&   .902&   .940
                                      &  .052&   .899&   .876&   .916 \\

$DSA2F_{21}$ \cite{sun2021deep}& - & .021 & .896 & .920  &.962 & .024 & .897 & .918  &.950 & .039 & .901 & .903  &.923 & .036 & .898 & .904  &.933 & - & - & -  &- \\%& .045 & .852 & .846  &.904 \\
%$DFMNet_{21}$ \cite{Zhang2021DFMNet}& 93 & .019 & .932 & .938  &.973 & .024 & .912 & .926  &.961 & .039 & .913 & .912  &.950 & .040 & .904 &.908  &.948 & .049 & .890 & .885  &.926 \\%& - & - & -  & - \\




%$TriTrans_{21}$ & \underline{.014} & .946 & .943  &.978 & .020 & .930 & .928  &.963 & .030 & .934 & .920  &.953 & \bl{.033} & .920 & .908  &.949 & \bl{.043} & 916 & .886  &.928  \\ %& - & - & -  & - \\

%$CMINet_{21}$ \cite{cascaded_cmi} & 818 & .016 & .944 & .940  &.975 & .020 & \bl{.931& \bl{.932  &.959 & .028 & \bl{.940& \bl{.929 & .954 & .032 & .925 & .918 &.946 & .040 & .923 & .898  &.934 \\%& - & - & -  & - \\

$DSNet_{21}$ \cite{wen2021dynamic} & 661& .021 & .939  & .928 & .956 & .024 & .925 & .926 & .951 & .034 & .929 & .921 &.946 & .036 & .922 & \bl{.914} & .941 & .052 & .899 & .876 & .910\\ 


$UTANet_{21}$ \cite{zhao2021rgb} & 186 & .026 & .921 & .900  &.932 & \bl{.020} & .928 & \bl{.932}  &\bl{.964} & .037 & .915 & .902  &.945 & .033 & .921 & .910  &.948 &.048 & .897 & .873  &.925 \\%& .042 & .881 & .885  &- \\


$C2DFNet_{22}$ \cite{zhang2022c} & 198& .020 & .937 & .922 & .948   &.021 & .926 & .928 & .956 & - & -& -& - & .038 & .911 & .902 & .938 & .053 & .894 & .782 & .911\\ 


$MVSalNet_{22}$ \cite{zhou2022mvsalnet}   & - & .019 & .942& .937& .973  &  .022&   .931&   .930&   .960 &  .036&   .923&   .912&   .944  &  .036&   .921&   .913&   .944 & - & - &- &-\\  

$SPSN_{22}$ \cite{lee2022spsn}  & 149 & .017 & .942& .937& .973 &  .023&   .917&   .923&   .956  &  .032&   .927&   .918&   .949 &  .035&   .909&   .906&   .941  &  .043&   .910&   .891&   .932 \\   

                                      
\rowcolor[RGB]{235,235,250} 

\textbf{Ours (ResNet50)} & 523 & \bl{.013} & \bl{.954} & \bl{.947} & \bl{.982} & \bl{.020} & .927 & .930 & .962 & \bl{.028} & \bl{.937} & \bl{.926} & \bl{.956} & \bl{.032} & \bl{.923} & \bl{.914} & \bl{.949} & \bl{.039} & \bl{.918} & \bl{.897} & \bl{.935} \\
\hline
\multicolumn{15}{l}{\textbf{Performance of RGB-D Models with Res2Net Backbones}}  \\
$SPNet_{21}$ \cite{zhouiccvspnet}& 702& \bl{.014} & \bl{.950} & \bl{.945}  & \bl{.980} &  .021 &  .925 &  .927  &.959 & \bl{.028} & \bl{.935} & \bl{.925}  &\bl{.954} & .037 & .915 & .907  &.944 & .043 & .916 & .894  &.930 \\ % & .044 & .883 & .871  & .915 \\

%$RFNet_{22}$ & 365 &.015& .946& .941& .977
%&\textbf{.020}&\textbf{.932}&\textbf{.931}&\textbf{.962}
%& .029 & .936 &\textbf{.926}& .951 
%&\textbf{.035}&\textbf{.921}&\textbf{.911}& .944 
%&\textbf{.042}& .916 & .893 &\textbf{.931} \\

\rowcolor[RGB]{235,235,250} 

%\textbf{Ours (Res2Net50)}&  525 & \bl{.013} & \bl{.952} & \bl{.946}  &\bl{.980} & \bl{.021} & \bl{.929} & \bl{.930}  &\bl{.961} &  .029 & \bl{.939} & \bl{.926}  &\bl{.954} & \bl{.035} & \bl{.921} & \bl{.911}  &\bl{.946} & \bl{.043} & \bl{.919} &  .892  & .927\\

  %\textbf{Ours (Res2Net50)}&  525 & .013 & .951 &.944 & .982 & .020 & .929 & .930 &.963 & .030 & .927 & .920 & .949 & .037 & .912 & .902 & .941 & .038 & .923 & .900 & .939 \\
  
 %\textbf{Ours (Res2Net50)}&  525 & .015 & .947 &.939 & .972 & .020 & .931 & .931 &.962 & .031 & .929 & .920 & .950 & .034 & .921 & .914 & .946 & .042 & .916 & .895 & .932 \\

 \textbf{Ours (Res2Net50)}&  525 & .017 & .947 &.935 & .965 & \bl{.019} & \bl{.935} & \bl{.934} &\bl{.967} & .031 & .930 & .922 & .950 & \bl{.036} & \bl{.917} & \bl{.908} & \bl{.944} & \bl{.038} & \bl{.925} & \bl{.902} & \bl{.939} \\


%\textbf{Ours (Res2Net50)}&  525 & .013 & .953 &.946 & .982 & .019 & .933 & .933 &.965 & .030 & .929 & .921 & .952 & .036 & .919 & .908 & .943 & .043 & .922 & .894& .932 \\


%\textbf{Ours (Res2Net50)}&  525 & .018 & .944 &.931 & .964 & .020 & .932 & .931 &.962 & .035 & .926 & .915 & .943 & .035 & .922 & .913 & .946 & .041 & .923 & .898& .935 \\


\hline

%$Ours (ResNet50) $ & .016 & .946 &.941 & .976  & \underline{.021} & \bl{.929} & \underline{.929}  &\underline{.961} & .030 & .934 & .922  &.952 & .037 & \underline{.916} & .906  &.941 & \underline{.044} & \underline{.916} & \underline{.892}  &.926 \\ 


%$Ours (Res50)$& 523 & .013 & .954 & .946 & .981 &.019 & .931 & .931 & .962 & .027 & .938 & .928 & .958 & .033 & .923 & .913 & .947 & .045 & .912 & .887 & .925 \\
%$Ours (Res50)$& 523 & .015 & .951 & .940 & .973 &.020 & .932 & .932 & .963 & .028 & .937 & .926 & .955 & .033 & .925 & .914 & .949 & .041 & .918 & .896 & .933 \\

 %& \bl{.047} & \bl{.873} & \bl{.871}  & \bl{.910} \\

%$Ours$ & \bl{.014} & \bl{.949} & \bl{.943}  &\bl{.979} & \bl{.020} & \bl{.931} & \bl{.931}  &\bl{.963} & \bl{.030} & \bl{.933} & \bl{.923}  &\bl{.951} & \bl{.034} & \bl{.921} & \bl{.912}  &\bl{.947} & \bl{.042} & \bl{.921} & \bl{.897}  &\bl{.932} & \bl{.041} & \bl{.885} & \bl{.882}  & \bl{.920} \\

%$Ours$ & \bl{.014} & \bl{.951} & \bl{.943}  &\bl{.980} & \bl{.019} & \bl{.929} & \bl{.930}  &\bl{.963} & \bl{.029} & \bl{.934} & \bl{.923}  &\bl{.952} & \bl{.035} & \bl{.918} & \bl{.908}  &\bl{.945} & \bl{.043} & \bl{.914} & \bl{.891}  &\bl{.927} & \bl{.042} & \bl{.881} & \bl{.874}  & \bl{.924} \\
 \hline 

\hline

\hline
\end{tabular*}
\end{center}

\end{table*}







\begin{table*}[t]
\scriptsize
\setlength\tabcolsep{4.3pt}
\setlength\extrarowheight{1pt}
\begin{center}
\caption{\textbf{Quantitative comparison} with SOTA models. $\uparrow$ ($\downarrow$) denotes that the higher (lower) is better. (\bl{Bold}: best.)}
\label{tab:quant}
\begin{tabular*}{\linewidth}{ll|| llll|llll|llll|llll||llll}
 \hline 

\hline

\hline
 Dataset &Size & \multicolumn{4}{c}{NLPR}  & \multicolumn{4}{c}{NJU2K}  & \multicolumn{4}{c}{STERE} & \multicolumn{4}{c}{SIP}  &\multicolumn{4}{c}{Average}  \\ %& \multicolumn{4}{c}{SSD} \\
\cline{3-6} \cline{7-10} \cline{11-14} \cline{15-18} \cline{19-22} %\cline{22-25}

Metric & (Mb) & $M\downarrow$ &  $F_{\beta}\uparrow $  &  $S_m\uparrow$ &  $E_m\uparrow$  &  $M\downarrow$ &  $F_{\beta}\uparrow $  &  $S_m\uparrow$ &  $E_m\uparrow$  &  $M\downarrow$ &  $F_{\beta}\uparrow $  &  $S_m\uparrow$ &  $E_m\uparrow$  &  $M\downarrow$ &  $F_{\beta}\uparrow $  &  $S_m\uparrow$ &  $E_m\uparrow$  &  $M\downarrow$ &  $F_{\beta}\uparrow $  &  $S_m\uparrow$ &  $E_m\uparrow$  \\%&  $M\downarrow$ &  $F_{\beta}\uparrow $  &  $S\uparrow$ &  $E\uparrow$\\
\hline
%$CPFP_{19}$ & .038 & .846 & .872  &.923 & .036 & .867 & .888  &.932 & .053 & .877 & .878  &.923 & .051 & .874 & .879  &.925 & .064 & .851 & .850  &.903 \\%& .082 & .766 & .807  &.852 \\

\multicolumn{15}{l}{\textbf{Performance of RGB-D Models with VGG Backbones}} \\

$DMRA_{19}$ \cite{piao2019dmra} & 278 & .031 & .888 & .899 &.940 
                                & .051 & .896 & .886 &.920 
                                & .047 & .895 & .886 &.930
                                & .086 & .852 & .806 &.847& .059 & .880 & .860 &.901  \\% & .058 & .844 & .857  &.906 \\
$A2dele_{20}$ \cite{piao2020a2dele} & 116 & .029 & .895 & .899  &.943 & .051 & .890 & .871  &.914 & .044 & .892 & .879  &.926 & .070 & .856 & .829  &.887 & .052 & .880 & .863  &.912 \\%& .070 & .776 & .802  &.861 \\

$ATSA_{20}$ \cite{zhang2020asymmetric}& 131   & .027 & .907 & .909  &.947 & .046 & .905 & .885  &.928 & .038 & .912 & .896  &\textbf{.940} & .063 & .884 & .849  &.895 & .046 & .901 & .879  &.923 \\%& .070 & .776 & .802  &.861 \\

$CMMS_{20}$ \cite{li2020rgb}& 546 & .028 & .914 & .919  &.946 & .044 & .905 & .900  &.929 & .045 & .899 & .894  &.925 & .058 & .893 & .872  &.901  & .047  & .900 & .890  &.920  \\%& .046 & .874 & .864  &.922 \\
$DANet_{20}$ \cite{zhao2020single}& 128  & .047 & .904 & .897 &.926 
                                & .045 & .910 & .899 & .927
                                & .048 & .895 & .892 &.919 
                                & .054 & .900 & .888 &.912 & .049 & .900 & .892 &.919 \\%& .050 & .866 & .864  &.914 \\


$CMWNet_{20}$ \cite{li2020cross}  & 327 & .029 & .913 & .917  &.941 & .046 & .913 & .903  &.925 & .043 & .911 & .905  &.930 & .062 & .889 & .867  &.901  &.048 & .904 &.893 & .920  \\%& .068 & .795 & .830  &.885 \\

$HDFNet_{20}$ \cite{pang2020hierarchical}& 308  & .023 & .926 & .923  &.957 & .039 & .922 & .908  &.939 & .042 & .910 & .900  &.933 &.048 & \textbf{.909} & .886  &.924 & .041 & .914 & .899  &.933  \\%& .048 & .808 & .866  &.913\\                      

$PGAR_{20}$ \cite{chen2020progressively}& 62 & .027 & .912 & .917  &.941 & .042 & .918 & .909  &.932 & .045 & .902 & .894  &.919 &.072 & .852 & .838  &.875 & .051 & .889 & .880  &.909    \\%& .048 & .808 & .866  &.913\\      

$SSF_{20}$ \cite{zhang2020select} & 126 & .027 & .912 & .915  &.947 & .043 & .911 & .899  &.929 & .065 & .859 & .837  &.882 &.091 & .810 & .799  &.855 & .065 & .858 & .844  &.889  \\%& .048 & .808 & .866  &.913\\

$CASGNN_{20}$ \cite{luo2020cascade}& 160  & .025 & .914 & .919  &.953 & .036 & .927 & .910  &.944 & \textbf{.038} & .913 & .899  &\textbf{.940} & -& - & -  &-  & - & - & -  &- \\%& .044 & .859 & .882  &.919 \\



$D3Net_{21}$ \cite{fan2019rethinkingd3}& 518  & .030 & .907 & .912 &.942 
                                & .049 & .910 & .900 &.928 
                                & .039 & .911 & .902 &\textbf{.940} 
                                & .063 & .886 & .866 &.897 & .048 & .902 & .890  &.923 \\%& .058 & .834 & .857  &.910 \\
$CDINet_{21}$ \cite{CDINet} & 217  & .024 & .923 & .927 &.953 
                                & \textbf{.030} & .928 & \textbf{.918} &.945 
                                & .040 & .912 & \textbf{.913} &.937 
                                & .054 & .904 & .875 &.908 & .041 & .913 & .903 &.930  \\%& - & - & -  & - \\

$UCNet_{21}$ \cite{zhang2021uncertainty} & 120 &.025 & .915 & .920 & .953 & .043 & .908 & .897 & .932 & .039 & .908 & .902 &.938 & .051 & .896 & .875 & .915 & .042 & .905 & .894 & .931 \\ 
$DRLF_{21}$ \cite{wang2020data} & 351 & .032 & .904 & .903  &.929 & .055 & .896 & .886  &.914 & .050 & .897 & .888  &.916 & .071 & .869 & .850  &.882 & .056 & .888 & .876  &.905 \\%& .068 & .795 & .830  &.885 \\
$HAINet_{21}$ \cite{li2021hierarchical}  & 228 &  .024&   .920&   .924&   .956 
                                      &  .037&   .924&   .911&   .940
                                      &  .040&   \textbf{.917}&   .907&   .938 
                                      &  .052&   .907&   .879&   .917 & .041 & .915 & .901  &.930 \\

$BIANet_{21}$ \cite{zhang2021bilateral} & 189  & .025 & .921 & .925  &.954 & .039 & .928 & .915  &.939 & .043 & .910 & .903  &.932 & .052 & .904 & .883  &.916 & .043 & .912 & .900  &.930\\%& .068 & .795 & .830  &.885 \\

$DCMF_{22}$ \cite{wang2022learning} & 78 &.029 & .913 & .922 & .940 & .041  & .911 &  .902 & .935 & .043 & .916 & .910 & .928 & - & -& -& - & - & - & - & - \\ 

\rowcolor[RGB]{235,235,250} 
\textbf{Ours (VGG16)} & 269 &\textbf{.021} & \textbf{.927} & \textbf{.928} & \textbf{.962} & .034 & \textbf{.930 }& \textbf{.918} & \textbf{.947} & .039 & .915 & .902 & .939 & \textbf{.045} & \textbf{.909} & \textbf{.889} & \textbf{.927} & \textbf{.038} & \textbf{.917} & \textbf{.903} & \textbf{.939 }  \\

\hline
\multicolumn{15}{l}{\textbf{Performance of RGB-D Models with ResNet Backbones}} \\
$JLDCF_{21}$ \cite{fu2021siamese} & 548 & .022 & .925 & .925  &.955 & .041 & .912 & .902  &.936 & .040 & .913 & .903  &.934 & .049 & .903 & .880  &.918 & .041 & .911 & .897  &.931 \\%& .068 & .795 & .830  &.885 \\

$RD3D_{21}$ \cite{chen2021rgb}  & 179 & .022 & .927 & .930  &.959 & .036 & .923 & .916  &.941 & .037 &.917 & .911  &.939 & .048 & .906 & .885  &.918& .038 & .915 & .905  &.934 \\%& .068 & .795 & .830  &.885 \\


$BIANet_{21}$ \cite{zhang2021bilateral} & 244 & .023 & .924 & .926  &.956 & .036 & .929 & .917  &.942 & .039 & .912 & .905  &.935 & .047 & .904 & .887  &.920 & .039 & .914 & .903  &.933 \\%& .068 & .795 & .830  &.885 \\


$CoNet_{20}$ \cite{ji2020accurate}& 162 & .027 & .903 & .911  &.943 & .046 & .902 & .896  &.926 & .037 & .909 & .905  &.941 & .058 & .887 & .860  &.911 & .045 & .900 & .889  &.928 \\% & .059 & .840 & .853  &.915 \\

$DASNet_{20}$ \cite{zhao2020depth} & 141  & .021 & \bl{.929} & .929  &.960 & .042 & .911 & .902  &.935 & .036 & .915 & .910  &.939 &.051 & .900 & .877  &.918 & .040 & .911 & .899  &.933\\%& .042 & .881 & .885  &- \\


$BBSNet_{21}$ \cite{zhai2021bifurcated}& 200 & .023 & .927 & .930  &.953 & .035 & .931 & .920  &.941 & .041 & .919 & .908  &.931 &.055 & .902 & .879  &.910 & .043 & .916 & .903  &.928 \\%& .044 & .859 & .882  &.919 \\

$DCF_{21}$ \cite{ji2021calibrated} & 435    &  .022&   .918&   .924&   .958
                                      &  .036&   .922&   .912&   .946
                                      &  .039&   .911&   .902&   .940
                                      &  .052&   .899&   .876&   .916 & .041 &.910 & .897 &.935\\

$DSA2F_{21}$ \cite{sun2021deep}& -  & .024 & .897 & .918  &.950 & .039 & .901 & .903  &.923 & .038 & .910 & .898  &.939 & .057 & 
.891& .862  &.908 & .043 & .900 & .889  &.927\\%& .045 & .852 & .846  &.904 \\
%$DFMNet_{21}$ \cite{Zhang2021DFMNet}& 93 & .019 & .932 & .938  &.973 & .024 & .912 & .926  &.961 & .039 & .913 & .912  &.950 & .040 & .904 &.908  &.948 & .049 & .890 & .885  &.926 \\%& - & - & -  & - \\




%$TriTrans_{21}$ & \underline{.014} & .946 & .943  &.978 & .020 & .930 & .928  &.963 & .030 & .934 & .920  &.953 & \bl{.033} & .920 & .908  &.949 & \bl{.043} & 916 & .886  &.928  \\ %& - & - & -  & - \\

%$CMINet_{21}$ \cite{cascaded_cmi} & 818 & .016 & .944 & .940  &.975 & .020 & \bl{.931& \bl{.932  &.959 & .028 & \bl{.940& \bl{.929 & .954 & .032 & .925 & .918 &.946 & .040 & .923 & .898  &.934 \\%& - & - & -  & - \\

$DSNet_{21}$ \cite{wen2021dynamic} & 661& .024 & .925 & .926 & .951 & .034 & .929 & .921 &.946 & .036 & .922 & \bl{.914} & .941 & .052 & .899 & .876 & .910 & .039 & .916  & .904 & .932 \\ 


$UTANet_{21}$ \cite{zhao2021rgb} & 186 & \bl{.020} & .928 & \bl{.932}  &\bl{.964} & .037 & .915 & .902  &.945 & .032 & .921 & .910  &.948 &.048 & .897 & .873  &.925 & .037 & .913 & .898  &.941  \\%& .042 & .881 & .885  &- \\


$C2DFNet_{22}$ \cite{zhang2022c} & 198  &.021 & .926 & .928 & .956 & - & -& -& - & .038 & .911 & .902 & .938 & .053 & .894 & .872 & .911 & - & - & - & - \\ 
%

$MVSalNet_{22}$ \cite{zhou2022mvsalnet}   & - &  .022&   .931&   .930&   .960 &  .036&   .923&   .912&   .944  &  .036&   .921&   .913&   .944 & - & - &- &-  & - & -& -& - \\  

$SPSN_{22}$ \cite{lee2022spsn}  & 149 &  .023&   .917&   .923&   .956  &  .032&   .927&   .918&   .949 &  .035&   .909&   .906&   .941  &  .043&   .910&   .891&   .932 & .036 & .914& .905& .941  \\   

                                      
\rowcolor[RGB]{235,235,250} 

\textbf{Ours (ResNet50)} & 523 & \bl{.020} & .927 & .930 & .962 & \bl{.028} & \bl{.937} & \bl{.926} & \bl{.956} & \bl{.032} & \bl{.923} & \bl{.914} & \bl{.949} & \bl{.039} & \bl{.918} & \bl{.897} & \bl{.935} & \bl{.032} & \bl{.924} & \bl{.912} & \bl{.947} \\
\hline
\multicolumn{15}{l}{\textbf{Performance of RGB-D Models with Res2Net Backbones}}  \\

$BIANet_{21}$ \cite{zhang2021bilateral} & 244& .022 & .926 & .928  &.957 & .034 & .932 & .923  &.945 & .038 & .916 & .908  &.935 & .046 & .908 & .889  &.922  & .038 & .917 & .906  &.935 \\%& .068 & .795 & .830  &.885 \\


$SPNet_{21}$ \cite{zhouiccvspnet}& 702 &  .021 &  .925 &  .927  &.959 & \bl{.028} & \bl{.935} & \bl{.925}  &\bl{.954} & .037 & .915 & .907  &.944 & .043 & .916 & .894  &.930 & .035 & .920& .908  & .943 \\ % & .044 & .883 & .871  & .915 \\

%$RFNet_{22}$ & 365 &.015& .946& .941& .977
%&\textbf{.020}&\textbf{.932}&\textbf{.931}&\textbf{.962}
%& .029 & .936 &\textbf{.926}& .951 
%&\textbf{.035}&\textbf{.921}&\textbf{.911}& .944 
%&\textbf{.042}& .916 & .893 &\textbf{.931} \\

\rowcolor[RGB]{235,235,250} 

%\textbf{Ours (Res2Net50)}&  525 & \bl{.013} & \bl{.952} & \bl{.946}  &\bl{.980} & \bl{.021} & \bl{.929} & \bl{.930}  &\bl{.961} &  .029 & \bl{.939} & \bl{.926}  &\bl{.954} & \bl{.035} & \bl{.921} & \bl{.911}  &\bl{.946} & \bl{.043} & \bl{.919} &  .892  & .927\\

  %\textbf{Ours (Res2Net50)}&  525 & .013 & .951 &.944 & .982 & .020 & .929 & .930 &.963 & .030 & .927 & .920 & .949 & .037 & .912 & .902 & .941 & .038 & .923 & .900 & .939 \\
  
 %\textbf{Ours (Res2Net50)}&  525 & .015 & .947 &.939 & .972 & .020 & .931 & .931 &.962 & .031 & .929 & .920 & .950 & .034 & .921 & .914 & .946 & .042 & .916 & .895 & .932 \\

 \textbf{Ours (Res2Net50)}&  525& \bl{.019} & \bl{.935} & \bl{.934} &\bl{.967} & .031 & .930 & .922 & .950 & \bl{.036} & \bl{.917} & \bl{.908} & \bl{.944} & \bl{.038} & \bl{.925} & \bl{.902} & \bl{.939}  & \textbf{.033} & \textbf{.924} &\textbf{.911} & \textbf{.946} \\


%\textbf{Ours (Res2Net50)}&  525 & .013 & .953 &.946 & .982 & .019 & .933 & .933 &.965 & .030 & .929 & .921 & .952 & .036 & .919 & .908 & .943 & .043 & .922 & .894& .932 \\


%\textbf{Ours (Res2Net50)}&  525 & .018 & .944 &.931 & .964 & .020 & .932 & .931 &.962 & .035 & .926 & .915 & .943 & .035 & .922 & .913 & .946 & .041 & .923 & .898& .935 \\


\hline

%$Ours (ResNet50) $ & .016 & .946 &.941 & .976  & \underline{.021} & \bl{.929} & \underline{.929}  &\underline{.961} & .030 & .934 & .922  &.952 & .037 & \underline{.916} & .906  &.941 & \underline{.044} & \underline{.916} & \underline{.892}  &.926 \\ 


%$Ours (Res50)$& 523 & .013 & .954 & .946 & .981 &.019 & .931 & .931 & .962 & .027 & .938 & .928 & .958 & .033 & .923 & .913 & .947 & .045 & .912 & .887 & .925 \\
%$Ours (Res50)$& 523 & .015 & .951 & .940 & .973 &.020 & .932 & .932 & .963 & .028 & .937 & .926 & .955 & .033 & .925 & .914 & .949 & .041 & .918 & .896 & .933 \\

 %& \bl{.047} & \bl{.873} & \bl{.871}  & \bl{.910} \\

%$Ours$ & \bl{.014} & \bl{.949} & \bl{.943}  &\bl{.979} & \bl{.020} & \bl{.931} & \bl{.931}  &\bl{.963} & \bl{.030} & \bl{.933} & \bl{.923}  &\bl{.951} & \bl{.034} & \bl{.921} & \bl{.912}  &\bl{.947} & \bl{.042} & \bl{.921} & \bl{.897}  &\bl{.932} & \bl{.041} & \bl{.885} & \bl{.882}  & \bl{.920} \\

%$Ours$ & \bl{.014} & \bl{.951} & \bl{.943}  &\bl{.980} & \bl{.019} & \bl{.929} & \bl{.930}  &\bl{.963} & \bl{.029} & \bl{.934} & \bl{.923}  &\bl{.952} & \bl{.035} & \bl{.918} & \bl{.908}  &\bl{.945} & \bl{.043} & \bl{.914} & \bl{.891}  &\bl{.927} & \bl{.042} & \bl{.881} & \bl{.874}  & \bl{.924} \\
 \hline 

\hline

\hline
\end{tabular*}
\end{center}

\end{table*}
